Climbing the SkyLadder: A Certified Lower Bound of 25 for Kochen-Specker Sets in $\mathbb{R}^3$

Can an AI agent find new techniques for a search problem that experts already optimised? Can we trust a "no" answer that the agent's own code produced? We introduce SkyLadder, a protocol for agent-driven research on exact search problems. The agent climbs the problem one size at a time. It develops techniques motivated by measured bottlenecks and records both improvements and dead ends. Certification requires complete coverage by certificate checkers that Lean 4 proves sound. We apply SkyLadder to the minimum Kochen-Specker (KS) problem in $\mathbb{R}^3$, a question from the foundations of quantum mechanics. The best lower bound was 24 vectors. It came from two independent SAT-based searches of about 12,000 CPU-hours each. On one 8-core laptop, the agent's pipeline reproduces every published order from 17 to 23 and matches the published candidate counts exactly. At order 23 it is $2.5\times10^{4}$ times faster than the state of the art. Most of the gain comes from one reformulation: the search runs over basis structures instead of vector graphs. The pipeline resolves the next open case: every KS set in $\mathbb{R}^3$ has at least 25 vectors. The certificate checks establish that the enumeration is complete. They cover 2.2 million final basis structures across orders 1-24 and validate 1,027 real-algebraic non-embeddability certificates. The retained verification records account for all 1,748,733 required order-24 structures, including supplementary and cube-split checks. Lean proves that the checkers are sound. The trusted base also includes the mathematical specification, Lean and Mathlib, compiled checker execution, certificate-file handling, and assembly of per-process logs. Under this explicit trusted base, the result does not depend on the correctness of the search tools. An ablation and a prior-art audit separate the new techniques from those that the agent rediscovered.

==> figs/order_panels.tex <==
\begin{minipage}[t]{.325\linewidth}\centering\resizebox{\linewidth}{!}{\obp{orders 1--16}{$\le$11}{722}{40{,}333}{287}{287}{0}{$L^\ast$}{enum 6.51\,s, checks 2.11\,s}}\end{minipage}\hfill
\begin{minipage}[t]{.325\linewidth}\centering\resizebox{\linewidth}{!}{\obp{order 17}{12}{598}{36{,}524}{310}{310}{0}{$L^\ast$ (1{,}105)}{enum 9.49\,s, checks 3.25\,s}}\end{minipage}\hfill
\begin{minipage}[t]{.325\linewidth}\centering\resizebox{\linewidth}{!}{\obp{order 18}{13}{1{,}248}{75{,}089}{650}{650}{0}{$L^\ast$ (1{,}105)}{enum 25\,s, checks 8.66\,s}}\end{minipage}\\[3mm]
\begin{minipage}[t]{.325\linewidth}\centering\resizebox{\linewidth}{!}{\obp{order 19}{14}{3{,}153}{169{,}659}{1{,}905}{1{,}905}{0}{$L^\ast$ (1{,}105)}{enum 72\,s, checks 30\,s}}\end{minipage}\hfill
\begin{minipage}[t]{.325\linewidth}\centering\resizebox{\linewidth}{!}{\obp{order 20}{15}{8{,}576}{416{,}167}{5{,}423}{5{,}423}{0}{$L^\ast$ (1{,}105)}{enum 244\,s, checks 100\,s}}\end{minipage}\hfill
\begin{minipage}[t]{.325\linewidth}\centering\resizebox{\linewidth}{!}{\obp{order 21}{16}{28{,}196}{1{,}178{,}952}{19{,}620}{19{,}620}{0}{$L^\ast$ (1{,}105)}{enum 258\,s, checks 421\,s}}\end{minipage}\\[3mm]
\begin{minipage}[t]{.325\linewidth}\centering\resizebox{\linewidth}{!}{\obp{order 22}{17}{104{,}388}{3{,}826{,}507}{76{,}192}{76{,}192}{0}{$L^\ast$ (1{,}105)}{enum 819\,s, checks 1{,}772\,s}}\end{minipage}\hfill
\begin{minipage}[t]{.325\linewidth}\centering\resizebox{\linewidth}{!}{\obp{order 23}{18}{451{,}577}{14{,}705{,}862}{347{,}189}{347{,}188}{1 (1{,}665 cubes)}{$L^\ast$ (1{,}105)}{enum 5{,}083\,s, checks 23{,}839\,s}}\end{minipage}\hfill
\begin{minipage}[t]{.325\linewidth}\centering\resizebox{\linewidth}{!}{\obp{order 24}{19}{2{,}200{,}310}{65{,}833{,}376}{1{,}748{,}733}{1{,}748{,}668}{65 (45{,}870 cubes)}{$L^{\ast\ast}$ (1{,}107)}{enum 17{,}098\,s, checks 122{,}595\,s}}\end{minipage}\hfill

